Precedence thinness in graphs

Interval and proper interval graphs are very well-known graph classes, for which there is a wide literature. As a consequence, some generalizations of interval graphs have been proposed, in which graphs in general are expressed in terms of $k$ interval graphs, by splitting the graph in some special way. As a recent example of such an approach, the classes of $k$-thin and proper $k$-thin graphs have been introduced generalizing interval and proper interval graphs, respectively. The complexity of the recognition of each of these classes is still open, even for fixed $k \geq 2$. In this work, we introduce a subclass of $k$-thin graphs (resp. proper $k$-thin graphs), called precedence $k$-thin graphs (resp. precedence proper $k$-thin graphs). Concerning partitioned precedence $k$-thin graphs, we present a polynomial time recognition algorithm based on $PQ$-trees. With respect to partitioned precedence proper $k$-thin graphs, we prove that the related recognition problem is \NP-complete for an arbitrary $k$ and polynomial-time solvable when $k$ is fixed. Moreover, we present a characterization for these classes based on threshold graphs.

==> sections/literature_review.tex <==
\section{Literature Review on Thinness in Graphs}\label{chpt:literature:review}

In this section, we present a literature review concerning thinness in graphs. %More specifically, how it compares to other graphs parameters,
Since the subject has very recently been introduced, this review  is mainly based on that presented in~\cite{Bono18} and the results presented in there. 

Firstly, we show how the thinness compares to other graph parameters. The first parameter is the boxicity~\cite{roberts69Box}. 
The \emph{boxicity} of a graph $G$, or \emph{$box(G)$}, consists of the smallest integer $k$ for which $G$  is a intersection graph on the family of axis-parallel boxes in a   $k$-dimensional space. In~\cite{Mannino_theindependent} it was proved that $box(G) \leq thin(G)$. Also, in the same work, it was noted that this bound is not tight due to the fact that the $(r \times r)$-grid has thinness $\Theta(n)$ and boxicity $2$.
%A \emph{($x \time y$)-grid} is <definição>.

A sequence $X_1 , \ldots, X_r$ of subsets of $V(G)$  is a \emph{path decomposition} of $G$ if the following conditions are satisfied: 
    \begin{itemize}
        \item for every  $e\in  E(G)$, some $X_i$, $1 \leq i \leq r$, contains both ends of $e$;
        \item for $1 \leq i \leq  i' \leq i'' \leq r$, $X_i \cap X_{i''} \subseteq X_{i'}$.
    \end{itemize}
The \emph{pathwidth}~\cite{pathwidth83} of a graph $G$, or \emph{$pathw(G)$}, is the minimum value of $k \geq 0$ such that $G$ has a path decomposition $X_1 , \ldots, X_r$ with $|X_i| \leq k+ 1$, $1 \leq i \leq r$. In~\cite{Carl07}, it is shown that $thin(G) \leq pathw(G)+1$. Moreover, it shows that  the difference between these parameters may be arbitrarily large since $pathw(K_n) = n-1$ and $thin(K_n) = 1$.

The \emph{linear MIM-width} of $G$  c.f.~\cite{Bono18}, denoted by \emph{$lmimw(G)$},  is the smallest integer $k$ such that $V(G)$ can be arranged in a linear layout $v_1, \ldots, v_n$ in such a way that, for all $1 \leq i \leq n-1$, the size of the maximum induced matching of $G[E']$ is $k$, where $E'= \{(u,v)\in E(G) \mid u\in\{v_1, \ldots, v_i\}\text{ and } v\in\{v_{i+1}, \ldots, v_n\}\}$. In~\cite{Bono18}, it is proved that $lmimw(G) \leq thin(G)$.

The \emph{cutwidth} of a graph $G$, or \emph{$cutw(G)$}, is the smallest integer $k$ such that $V(G)$ can be arranged in a linear layout $v_1, \ldots, v_n$ in such a way that, for all $1\leq i \leq n-1$, there are at most $k$ edges with one endpoint in $\{v_1,\ldots,v_i\}$ and the other in $\{v_{i+1},\ldots,v_n\}$. In~\cite{Bono18}, it is proved that the layout related to the cutwidth leads to a $(cutw(G)+1)$-partition of $V(G)$ for which there is a consistent ordering. Consequently, $thin(G) \leq cutw(G)+1$.
            
The \emph{vertex isoperimetric peak} of $G$  c.f.~\cite{Bono18}, or \emph{$b_v(G)$}, is defined as $$\max_s \min_{X \subset V,|X|=s} |N(X)|$$. In~\cite{Mannino_theindependent}, it is proved that $thin(G) \geq \frac{b_v(G)}{\Delta (G)}$.


We define $f$ as  a \emph{t-rainbow dominating function} of a graph $G$ if it assigns a subset $f(v)$ of $\{1, \ldots , t\}$ to each $v \in V(G)$ such that $\bigcup_{u \in N(v)} f(u) = \{1, \ldots , t\}$ for all  $v$ with $f(v) = \emptyset$. The \emph{$t$-rainbow domination problem} consists in determining a $t$-rainbow dominating function that minimizes $\sum_{v\in V(G)}|f(v)|$.


Regarding the thinness of graphs resulting from graph operations, in~\cite{Bono18}, it is shown some result relating the (proper) thinness of the resulting graph to the (proper) thinness of the graphs under operation. Let $G_1$ and $G_2$ be graphs such that $V(G_1) \cap V(G_2) = \emptyset$. It was proved that: 
\begin{itemize}
    \item $thin(G_1\; \cup \; G_2) = \max\{thin(G_1),thin(G_2)\}$
    
    
    \item  If $G_2$ is complete, then
$\thin(G_1\; \vee \; G_2) = \thin(G_1)$. Otherwise,  $\thin(G\; \vee \; 2K_1) = \thin(G)+1$ and $\thin(G_1\; \vee \; G_2) \leq \thin(G_1)+\thin(G_2)$.

    
    \item $thin(G_1 \; \square \; G_2) \leq
thin(G_1)|V(G_2)|$

\end{itemize}
All these results also hold for proper thinness. 
In special, the last result was employed to solve the $t$-rainbow domination problem in graphs with bounded thinness, for a fixed $t$.

Given an interval graph $G$, the \emph{interval count} $IC(G)$ of $G$~\cite{Leibowitz78,ceriolisurvey} is the minimum number of distinct interval lengths needed to an interval model of $G$. An interval graph $G$ is said to be a \emph{$k$-length interval} graph if $IC(G) \leq k$. An interval graph $G$ is a \emph{$k$-nested}~\cite{Klavik2019} graph if it has a model in which no $k+1$ intervals can be linearly ordered by set inclusion. The class of $k$-length graphs is a subclass of $k$-nested graphs.

Let $\overline{tK_2}$ be the complement of a matching of size $t$. We now present results concerning graph classes in general. In~\cite{Carl07}, it was shown that $thin(\overline{tK_2}) = t$, for all $t \geq 1$. In~\cite{Bono18}, it is proved the following results. For the class of interval graphs, the proper thinness parameter is unbounded.   
For a given cograph $G$, $thin(G) \leq t$ if, and only if,  $G$ does not contains  $\overline{(t+1)K_2}$ as an induced subgraph. The thinness of a complete $m$-ary tree is $\Theta(\log n)$. Considering other generalizations based on interval graphs, $k$-nested interval graphs are proper $k$-thin but, for $k \geq 3$, there are proper $3$-thin graphs that are not $k$-nested interval graphs.

Also in~\cite{Bono18}, it is presented an efficient algorithm to determine the minimum partition of $V(G)$ for which a given vertex ordering is (strongly) consistent. Moreover, it is  proved that the problem of determining the existence of a (strongly) consistent ordering for a given partition of $V(G)$ with an  arbitrary number of parts is $NP$-complete. Besides that,  the problem of determining the existence of a (strongly) consistent ordering for a given partition of $V(G)$ with an  fixed number of parts is open.
In general, even for a fixed $k \geq 2$, the complexity of deciding whether a graph is (proper) $k$-thin is still open. Additionally, a characterization based on forbidden subgraphs, for all $k\geq 2$, is also open.


==> sections/prelim-long.tex <==
\section{Preliminaries}\label{chpt:preliminaries}
In this section, we  describe all the necessary terminology to the understanding of this work.

\subsection{General graph theory terminology}

A \emph{graph} $G$ is a pair $(V,E)$ of sets. The set $V$ is named \emph{vertex set} and $E$ the \emph{edge set} of $G$. The set $E$ consists of pairs of elements of $V$. A graph represents a set of objects (vertices) and a pairwise mutual relation (edges). By convention, $V(G)$ and $E(G)$  are the vertex set  and the edge set of the graph $G$, respectively. Unless stated otherwise, $|V(G)| = n$ and $|E(G)| = m$. 

We say the pair of  vertices $u,v \in V(G)$ are \emph{adjacent} in $G$ if $(u,v) \in E(G)$.
A \emph{simple graph} is a graph in which no vertex is adjacent to itself and there are no two edges consisting of the same pair of vertices. 
In the context of this work, we refer to simple graphs simply as graphs. 
A vertex $u\in V(G)$ is said to be \emph{universal} (in $G$) if it is adjacent to all the other vertices of $G$. 
The \emph{complement} $\overline{G}$ of $G$ is the graph defined as $\overline{G} = (G(V),E')$, where $E' =  \{(u,v)\not \in E(G) \}$.

A \emph{matching} in a graph $G$ is a subset $E'\subseteq E(G)$ in which there are no $e_1,e_2 \in E'$ having a vertex in common. 
An \emph{induced matching} in a graph $G$ is a matching $E'$ of $G$ in which there are no  $e_1, e_2 \in E'$ such that an edge of $G$ has a common vertex to both $e_1$ and $e_2$ (that is, no edges of the matching can be ''linked'' by an edge) 

Two graphs $G$ and $H$ are said to be \emph{isomorphic}, denoted by $G \cong H$, if there is a bijection $\theta : V(G) \rightarrow V(H)$ such that $(u,v) \in E(G)$ if, and only if, $(\theta(u),\theta(v)) \in E(H)$.

Let $V' \subseteq V(G)$. The \emph{induced subgraph} of $G$ by $V'$, denoted by $G[V']$, is the graph $G[V']= (V',E')$, where  $E' =  \{ (u,v)\in E(G) \mid u, v \in V' \}$. Analogously, for some $E' \subseteq E(G)$, let  the \emph{induced subgraph} of $G$ by $E'$, denoted by $G[E']$, be the the graph $G[E']= (V',E')$, where  $V' =  \{ u, v \in V(G) \mid  (u,v)\in E' \}$. 
A graph $G'$ obtained from $G$ by \emph{removing} the vertex $v \in V(G)$ is defined as $G' = (V \setminus \{v\},  E')$, where $E'=\{(u,w) \in E \mid u \neq v \text{ and } w \neq v\}$ 

A \emph{path} of a graph $G$ is a sequence $v_1,v_2, \ldots,v_i$ of distinct vertices of $V(G)$, $1 \leq i \leq n$, such that for all $1 \leq j<i$, $v_j$ and $v_{j+1}$  are adjacent in $G$. The \emph{length} of a path $v_1,v_2, \ldots,v_i$ is defined as $i-1$.
The \emph{path} graph $P_n$ is a graph consisting of a unique path with length $n-1$. A \emph{cograph} $G$ is a graph in which there is no $V' \subseteq V(G)$ such that $G[V'] \cong P_4$.
A \emph{cycle} of a graph $G$ is a path $v_1,v_2, \ldots,v_i$ of $G$ in which $(v_1,v_i) \in E(G)$. A graph $G$ is \emph{connected} if for all $u, v \in V(G)$, there is a path $v_1, \ldots, v_i$ in $G$ such that $v_1 = u$ and $v_i = v$.

A $tree$ $T$ is a connected graph that has no cycles. A \emph{rooted tree} $T_v$ is a tree in which a vertex $v \in V(T)$ is labeled as the \emph{root} of the tree. All the other vertices, known as \emph{nodes} of $T_v$, have implicit positions in relation to the root. 
%The \emph{level} of a node $u$ of $T_v$, denoted by $l(u)$,  corresponds to the length of the path from $v$ to $u$.
Let $u,w \in V(T_v)$, $w$ is a \emph{descendant} of $u$ if the path from $w$ to $v$ includes $u$. The node $w$ is said to be a \emph{child} of $u$ if it is a descendant of $u$ and $(w,u) \in E(T_v)$. The \emph{children} of $u$ is defined as the set that containing all child nodes of $u$. The node $u$ is said to be a \emph{leaf} of $T_v$ if it has no child in $T_v$. 
The \emph{subtree} $T_u$ of $T_v$  \emph{rooted at} the node $u$ is the tree that consists of $u$ as the root  and its descendants in $T_v$.  


A subset $L \subseteq V(G)$ is called an \emph{independent set} of $G$ if, for all distinct $u,v \in L$, $(u, v) \not \in E(G)$.
The \emph{(open) neighborhood} of $u \in V(G)$ is $N_G(u) =  \{v \in V(G) \mid  (u, v) \in E(G) \}$. Let $U \subseteq V(G)$ and define $N_G(U) = \bigcup_{u \in U} N_G(u) \setminus U$. The \emph{(closed) neighborhood} of $u \in V(G)$ is  defined as $N_G[u] = N_G(u) \cup \{u\}$. Similarly, let $U \subseteq V(G)$, $N_G[U] = N_G(u) \cup \{u\}$.
When $G$ is clear in the context, it may be omitted from both notations.
We define  $u, v \in V(G)$ as \emph{false twins} if $N(u) = N(v)$.





A vertex subset $C \subseteq V(G)$ is a \emph{clique} (of $G$) if its vertices are pairwise adjacent in $G$. A clique $C$ is \emph{maximal} if there is no $v  \in V(G) \setminus C$ such that $C \cup \{v\}$ is a clique. A vertex $v \in V(G)$ is said to be \emph{simplicial} if $G[N(v)]$ is a clique. A \emph{complete graph} $K_n$ is a graph such that $|V(K_n)| = n$ and $V(K_n)$ is a clique. 


A \emph{directed graph}, or \emph{digraph}, is a graph $D = (V,E)$ such that $E$ consisted of by ordered pairs of $V(G)$. A \emph{directed cycle} of a digraph $D$ is a sequence $v_1,v_2, \ldots,v_i$, $1 \leq i \leq n$, of vertices of $V(D)$ such that $v_1 = v_i$ and, for all $1 \leq j<i$, $(v_j,v_{j+1}) \in E(D)$. A \emph{directed acyclic graph} (\emph{DAG}) $D$ is a digraph with no directed cycles.  A \emph{topological ordering} of a DAG $D$ is a sequence $v_1,v_2,\ldots ,v_n$ of $V(D)$ such that there are no $1\leq i <j\leq n$ such that $(v_j,v_i) \in E(D)$. Determining a topological ordering of a DAG can be solved in time $O(n)$.


Let $G_1$ and $G_2$ be graphs such that $V(G_1) \cap V(G_2) = \emptyset$. The \emph{union} $G_1 \cup G_2$  is defined as the graph $G = (V(G_1) \cup V(G_2), E(G_1) \cup E(G_2))$. The \emph{join} $G_1 \vee G_2$ is defined as the graph $G = (V(G_1) \cup V(G_2), E(G_1) \cup E(G_2)\cup V(G_1)\times V(G_2))$. The \emph{cartesian product} $G_1 \;\square\; G_2$ is defined as the graph $G = (V(G_1) \times V(G_2),E')$ where $E' = \{((u_1,u_2),(v_1,v_2)) \in V(G_1) \times V(G_2) \mid \text{either } [u_1 = v_1\text{ and } (u_2,v_2) \in E(G_2)] \text{ or } [u_2 = v_2\text{ and } (u_1,v_1) \in E(G_1)]\} $. 
The \emph{$(m\times n)$-grid} is $P_m \;\square\; P_n$.
%The \emph{neighborhood} of a vertex $u \in V(G)$, denoted by $N(u)$, is the set $\{ v \in V(G): (u,v) \in E(G)\}$. Let $N[u] = N(u) \cup \{u\}$. We say that $u, v \in V(G)$ are \emph{twins} if $N[u] = N[v]$. 

An \emph{ordering} $s$ of elements   of a set $\mathcal{C}$ consists of a sequence $e_1,e_2,\ldots,e_n$  of all elements of $\mathcal{C}$. We say that $e_i$ \emph{precedes} $e_j$ in $s$, denoted by $e_i < e_j$, if $i < j$. An ordered tuple $(a_1, a_2, ... a_k)$ of some elements of $\mathcal{C}$ is according to $s$ if, for all $1 \leq i < k$, if $a_i = e_j$ and $a_{i+1} = e_z$, then $j < z$. Given orderings $s_1$ and $s_2$, the ordering obtained by concatenating $s_1$ to $s_2$ is denoted by $s_1s_2$. We define $\bar{s}$ as the \emph{reversal} of $s$. That is, $\bar{s} = e_n,e_{n-1},\ldots,e_1$. If $\mathcal{C}$  consists of a vertex subset of a graph, we define $V(s)=\mathcal{C}$. 


\subsection{Interval Graphs}
The \emph{intersection graph} of a family $\mathcal{F}$ of sets is the graph $G$ such that $V(G) = \mathcal{F}$ and $S,T \in V(G)$ are adjacent if and only if $S \cap T \neq \emptyset$.
An \emph{interval graph} $G$ is the intersection graph of a family $\mathcal{R}$ of intervals of the real line; such a family is called an \emph{interval model}, or  a \emph{model}, of the graph. 
We say that $\mathcal{R}$ is associated to $G$ and vice-versa.
It  is worth  mentioning that an interval graph can be associated to several models but an interval model can be associated to a unique graph. 
Concerning interval graphs, there are some characterizations of them which are relevant to this work, which we present next.

\begin{theorem}[\cite{Olariu91}]\label{theo:can:ordering}
A graph $G$ is an interval graph if, and only if, there is an ordering $s$ of $V(G)$ such that, for any triple $(p,q,r)$ of $V(G)$ ordered according to $s$, if $(p,r) \in E(G)$, then $(q,r) \in E(G)$.
\end{theorem}

The ordering described in Theorem~\ref{theo:can:ordering} is said to be a \emph{canonical} ordering.
Figure~\ref{fig:canonico} depicts an interval graph in which the vertices are presented from left to right in one of its canonical orderings. 

\begin{figure}
\centering     %%% not \center
\subfigure[]{\label{fig:canonico}\includegraphics[width=64mm]{figures/preliminaries/qualiOrdCan.pdf}}
\hspace{0.45cm}
\subfigure[]{\label{fig:canonicoproprio}\includegraphics[width=64mm]{figures/preliminaries/qualiOrdCanP.pdf}}
\caption{(a) Canonical ordering and (b) proper canonical ordering.}
\end{figure}

Let $\mathcal{R}$ be an interval model of an interval graph $G$. Note that, if we  draw a vertical line that  intersects a subset of intervals in $\mathcal{R}$, then these intervals consist of a clique in $G$. This is true because they all contain the point in which this line traverses. Moreover, if the given line traverses a maximal set of intervals, then the corresponding clique is maximal. Figure~\ref{fig:model} depicts an interval model and its maximal cliques for the graph in Figure~\ref{fig:canonico}.
The following is a characterization of interval graphs in terms of the maximal cliques of the graph.



\begin{figure}[htb]
\centering     %%% not \center
\includegraphics[width=90mm]{figures/preliminaries/qualiModel.pdf}

\caption{ An interval model an the maximal cliques of the graph in Figure~\ref{fig:canonico}.}
\label{fig:model}
\end{figure}


\begin{theorem}[\cite{Roberts69}]\label{theo:clique:ordering}
A graph $G$ is an interval graph if, and only if, there is an ordering $s_C = C_1,C_2, \ldots, C_k$ of its maximal cliques such that if $v \in C_i \cap C_z$  with $1 \leq i \leq z \leq k$, then $v \in C_j$, for all $i \leq j \leq z$.
\end{theorem}

The ordering described in Theorem~\ref{theo:clique:ordering} is said to be a \emph{canonical clique} ordering. The ordering of the maximal cliques depicted in Figure~\ref{fig:model}, read from left to right, represents a canonical clique ordering.

A \emph{proper interval graph} is an interval graph that admits an interval model in which no interval properly contains another. There is a characterization of proper interval graphs which is 
similar to that presented in Theorem~\ref{theo:can:ordering}, as described next.

\begin{theorem}[\cite{Roberts69}]\label{theo:procan:ordering}
A graph $G$ is a proper interval graph if, and only if, there is an ordering $s$ of $V(G)$  such that, for any triple $(p,q,r)$ of $V(G)$ ordered according to $s$, if $(p,r) \in E(G)$, then $(p,q), (q,r) \in E(G)$.
\end{theorem}

The ordering specified in the previous theorem is defined as a \emph{proper canonical} ordering. The ordering of the vertices of the graph depicted in Figure~\ref{fig:canonicoproprio} from left to right is proper canonical. Note that a proper canonical ordering is also a canonical ordering.
An important property of proper canonical orderings is the following: 

\begin{lemma}[\cite{Roberts69}]
Let $G$ be a graph. If $G$ is connected, then a proper canonical ordering of $G$ is unique up to reversion and permutation of true twin vertices.
\end{lemma}

As a consequence, if $G$ is disconnected, since each component has a unique proper canonical ordering, then the canonical ordering of $G$ consists of a permutation of canonical orderings of each of those components. 

Let $s$ be an ordering of $V(G)$ and $s_C = C_1,C_2, \ldots, C_k$ an ordering of the maximal cliques of $G$. 
The sequence $s$ is said to be \emph{ordered according} to $s_C$ if for all $u,v \in V(G)$ such that $u<v$ in $s$, there are no $ 1\leq i <j \leq k$ such that $v \in C_i$, $v \not \in C_j$ and  $u \in C_j$. As an example, note that the canonical ordering of the Figure~\ref{fig:canonico} is ordered according to  the maximal clique ordering $s_C = C_1,C_2, \ldots, C_6$ of the Figure~\ref{fig:model}.
The following lemma relates the characterization of canonical orderings and canonical clique ordering.

\begin{lemma}\label{lemma:clique:canonical}
Let $G$ be a graph and $s$ be an ordering of $V(G)$.  The ordering $s$ is a canonical ordering of $V(G)$ if, and only if, $s$ is ordered according to a canonical clique ordering of $G$.
\end{lemma}

\begin{proof}
Consider $s_C$ a canonical clique ordering of $G$. We will show that is possible to build a canonical ordering $s$ from $s_C$, respecting its clique ordering. To achieve this, first start with an empty sequence $s$. Iteratively, for each element $X$ of the sequence $s_C$, choose all simplicial vertices of $X$, adding them to $s$ in any order and removing them from $G$. 
Note that some of the vertices of $X$ that were not removed from $G$, because they were not simplicial in $G$, now may be turned simplicial by the removal of vertices.
Clearly, at the end of the process, $s$ will contain all the vertices of $G$.
Suppose $s$ is not a canonical ordering, that is, there are $p,q,r \in V(G)$, $p<q<r$ in $s$, such that $(p,r) \in E(G)$ and $(q,r) \not \in E(G)$. 
Let $C_p$, $C_q$ and $C_r$ be the maximal cliques of $s_C$ being processed at moment $p$, $q$ and $r$ were choose, respectively.  Note that $C_p < C_q < C_r$ in $S_c$ and, as $C_p$ is the last maximal clique in $s_C$ that contains $p$ and $(p,r) \in E(G)$,  $r \in C_p$. Besides, as $(q,r) \not \in E(G)$, $r \not\in C_q$ . Therefore, $r \in C_p \cap C_r$ and $r \not\in C_q$. A contradiction with the fact that $s_C$ is a canonical clique ordering. Hence, $s$ is a canonical ordering.


Consider $s= v_1,v_2, \ldots, v_n$ be a canonical ordering of $G$. We prove by induction in $|V(G)| = n$ that $s$ is ordered according to a canonical clique ordering. Clearly, the statement is true for $n = 1$. Suppose that the statement is true for any  $1 \leq n'< n$.
Let $s'$ be the sequence obtained from $s$ by removing $v_n$. Clearly $s'$ is also a canonical ordering and, by the induction hypothesis, $s'$ is ordered according with  a canonical clique ordering $s'_C = C_1,C_2, \ldots, C_k$. Let $C_i$, with $1 \leq i \leq k$, be the first clique of $s'_C$ such that $v_n \in N(C_i)$. 
Let $C' _j = \{C_j \cap N(v_n)\} \cup \{v_n\}$, $i \leq j \leq k$.
Note that, as $s$ is a canonical ordering, for all $C_j$ of $s'_C$, $i < j \leq k$, $\{C_j \cap N(v_n)\}\cup \{v_n\}$ is a maximal clique of $G$. 
If $C_i \subseteq N(v_n)$, then  $s'_C = C_1,C_2, \ldots, C'_i,C'_{i+1}, \ldots, C'_k$ is a canonical clique ordering that matches $s$. Otherwise, $s'_C = C_1,C_2, \ldots, C_i,C'_i,C'_{i+1}, \ldots, C'_k$ is a canonical clique ordering that matches $s$. Therefore, $s$ is ordered according to a canonical clique ordering of $G$.

\end{proof}

\subsubsection {PQ trees}

A \emph{$PQ$ tree}~\cite{BOOTH76} $T$ is a data structure that describes a family $\mathcal{F}$ of permutations of elements from a given set $\mathcal{C}$. 
In this tree, the set of leaves is $\mathcal{C}$ and the permutation being represented by the tree is the sequence of the leaves from left to right. Regarding  internal nodes, they are classified into two types, the $P$ and the $Q$ nodes. 
An \emph{equivalent} $PQ$ tree $T'$ to $T$ is a tree obtained from $T$ by any sequence of consecutive transformations, each consisting of either permuting the children of a $P$ node, or reversing the children of a $Q$ node. The family $\mathcal{F}$ of permutations of elements from $\mathcal{C}$ represented by  $T$ is that of permutations corresponding to all equivalent $PQ$ trees to $T$. 

Graphically, in a $PQ$ tree, leaves and $P$ nodes are represented by circles and $Q$ nodes by rectangles. Figure~\ref{fig:PQT:exeOp} depicts the described operations. In Figure~\ref{fig:PQT:1}, we have a partial representation of a $PQ$ tree. Figure~\ref{fig:PQT:2} depicts an equivalent $PQ$ tree obtained from a permutation of children of a $P$ node of this tree and Figure~\ref{fig:PQT:3} exemplifies an equivalent $PQ$ tree from the reversion of the children of a $Q$ node. 

\begin{figure}[htb]
    \centering % <-- added
    \subfigure[]{\label{fig:PQT:1}\includegraphics[width=40mm]{figures/preliminaries/qualiEqPQT.pdf}}\hfil
    \subfigure[]{\label{fig:PQT:2}\includegraphics[width=40mm]{figures/preliminaries/qualiEqPQT1_1.pdf}}\\
    \subfigure[]{\label{fig:PQT:3}\includegraphics[width=40mm]{figures/preliminaries/qualiEqPQT2_1.pdf}}\\\
    
\caption{A $PQ$ tree (a) and an example of permutations (b) and reversions (c) of children of its nodes. }
\label{fig:PQT:exeOp}
\end{figure}
\clearpage

One of the applications from the seminal paper introducing $PQ$ trees is that of recognizing interval graphs. 
In such an application, each  leaf of the $PQ$ tree  is a maximal clique of an interval graph $G$ and the family of permutations the tree represents is precisely all the canonical clique orderings of $G$~\cite{BOOTH76}. A $PQ$ tree can be constructed from an interval graph in time $O(n+m)$~\cite{BOOTH76}. 
In this work we consider $PQ$-trees only in this context.

We will say that a  vertex belongs to a node of a $PQ$ tree if it belongs to any leaf that descends from this node. Figure~\ref{fig:pre:PQT} depicts a $PQ$ tree of the interval graph of Figure~\ref{fig:canonico} according to the maximal cliques in  Figure~\ref{fig:model}. The permutations implicitly represented by this  $PQ$ tree are:
\begin{itemize}
    \item $C_1,C_2,C_3,C_4,C_5,C_6$
    \item $C_1,C_2,C_3,C_4,C_6,C_5$
    \item $C_1,C_2,C_4,C_3,C_5,C_6$
    \item $C_1,C_2,C_4,C_3,C_6,C_5$
    \item $C_6,C_5,C_4,C_3,C_2,C_1$
    \item $C_5,C_6,C_4,C_3,C_2,C_1$
    \item $C_6,C_5,C_3,C_4,C_2,C_1$
    \item $C_5,C_6,C_3,C_4,C_2,C_1$
    
\end{itemize}


\begin{figure}[htb]
\centering     %%% not \center
\includegraphics[width=40mm]{figures/preliminaries/qualiPQT.pdf}
\caption{A $PQ$ tree of the interval graph of Figure~\ref{fig:canonico} according to the maximal cliques in  Figure~\ref{fig:model}.}
\label{fig:pre:PQT}
\end{figure}

\subsection {Thinness in Graphs}

A graph $G$ is called a \emph{$k$-thin graph} if there is a $k$-partition $(V_1,V_2 \ldots, V_k)$ of $V(G)$ and an ordering $s$ of $V(G)$ such that, for any triple $(p,q,r)$ of $V(G)$ ordered according to $s$, if $p$ and $q$ are in a same part $V_i$ and $(p,r) \in E(G)$, then $(q,r)\in E(G)$. An ordering and a partition satisfying that property are called \emph{consistent}. That is, a graph is  $k$-thin if there is an ordering consistent with some $k$-partition of its vertex set. 
The \emph{thinness} of $G$, or \emph{$thin(G)$}, is the minimum value $k$ for which $G$ is a $k$-thin graph. 

A graph $G$ is called a \emph{proper $k$-thin graph} if $G$ admits a $k$-partition $(V_1, \ldots, V_k)$ of $V(G)$ and an ordering $s$ of $V(G)$ consistent with the partition and, additionally, for which any triple $(p,q,r)$ of $V(G)$, ordered according to $s$, if $q$ and $r$ are in a same part $V_i$ and $(p,r) \in E(G)$, then $(p,q)\in E(G)$. Equivalently, an ordering $s$ of $V(G)$ such that $s$ and its reverse are consistent with the partition. Such an ordering and partition are called \emph{strongly consistent}.
The \emph{proper thinness} of $G$, or \emph{$pthin(G)$}, is the minimum value $k$ for which $G$ is a proper $k$-thin graph.

Figures~\ref{fig:c4thin} and~\ref{fig:c4pthin} depict two bipartitions of a graph (where the classes are represented by distinct colors) and two different vertex orderings. The ordering of Figure~\ref{fig:c4thin} is consistent with the corresponding partition but not strongly consistent, while the ordering of Figure~\ref{fig:c4pthin} is strongly consistent with the corresponding partition.  

Note that $k$-thin graphs (resp. proper $k$-thin graphs) generalize interval graphs (resp. proper interval graphs). The parameter $thin(G)$ (resp. $pthin(G)$) is in a way a measure of how far a graph is from being an interval graph (resp. proper interval graph). The $1$-thin graphs (resp. proper $1$-thin graphs) are the interval graphs (resp. proper interval graphs).  

For instance, consider the graph $C_4$. Since $C_4$ is not an interval graph, $thin(C_4) > 1$. Figure~\ref{fig:c4} proves that $thin(C_4) = pthin(C_4) = 2$.

A characterization of $k$-thin or proper $k$-thin graphs by forbidden induced subgraphs is only known for $k$-thin graphs within the class of cographs~\cite{Bono18}. Graphs with arbitrary large thinness were presented in~\cite{Carl07}, while in~\cite{Bono18} a family of interval graphs with arbitrary large proper thinness was used to show that the gap between thinness and proper thinness can be arbitrarily large. The relation of thinness and other width parameters of graphs like boxicity, pathwidth, cutwidth and mim-width was shown in~\cite{Carl07,Bono18}. 

Let $G$ be a graph and ${<}$ an ordering of its vertices. The graph $G_{<}$ has $V(G)$ as vertex set, and $E(G_{<})$ is such that for $v < w$, $(v,w) \in E(G_{<})$ if and only if there is a vertex $z$ in $G$ such that $v < w < z$, $(z,v) \in E(G)$ and $(z,w) \not \in E(G)$. 
Similarly, the graph $\tilde{G}_<$ has $V(G)$ as vertex set, and $E(\tilde{G}_{<})$ is such that for $v < w$, $(v,w) \in E(\tilde{G}_{<})$ if and only if either there is a vertex $z$ in $G$ such that $v < w < z$, $(z,v) \in E(G)$ and $(z,w) \not \in E(G)$ or there is a vertex $x$ in $G$ such that $x < v < w$, $(x,w) \in E(G)$ and $(x,v) \not \in E(G)$.

\begin{theorem}\label{thm:coloring-order}\cite{B-M-O-thin-tcs,Bono18} Given a graph $G$ and an ordering ${<}$ of its vertices, a partition of $V(G)$ is consistent (resp. strongly consistent) with the ordering ${<}$ if and only if it is a valid coloring of $G_{<}$ (resp. $\tilde{G}_<$). 
\end{theorem}


%The computational complexity of deciding whether a graph is $k$-thin, or proper $k$-thin, even for fixed $k \geq 2$, is still an open problem. However, on the one hand, given a vertex ordering, there are  polynomial time algorithms that compute a partition into a minimum number of classes that is consistent (resp. strongly consistent) with that ordering~\cite{B-M-O-thin-tcs,Bono18}. On the other hand, given a vertex partition, the problems of deciding the existence of a vertex ordering consistent (resp. strongly consistent) with that partition are \NP-complete~\cite{Bono18}.   
%Moved to the intro


%Section~\ref{chpt:literature:review} presents a  literature review about this topic. 

\begin{figure}[htb]
    \centering % <-- added
\subfigure[]{\label{fig:c4thin}\includegraphics[width=40mm]{figures/preliminaries/qualiC4thin.pdf}}\hfil
\subfigure[]{\label{fig:c4pthin}\includegraphics[width=40mm]{figures/preliminaries/qualiC4pthin.pdf}}\hfil

\caption{(a) A consistent ordering and a (b) strongly consistent ordering of $V(C_4)$, for the corresponding $2$-partitions.}
\label{fig:c4}
\end{figure}


\subsection {Precedence Thinness and Precedence Proper thinness in Graphs}

In this work, we consider a variation of the problems described in the last subsection by requiring that, given a vertex partition, the (strongly) consistent orderings hold an additional property. Next, we define the two graph classes deriving from this additional restriction. 

A graph $G$ is \emph{\fpExt{k}} (resp. \emph{\fppExt{k}}), or \emph{\fp{k}} (resp. \emph{\fpp{k}}), if there is a $k$-partition of its vertices and a  consistent (resp. strongly consistent) ordering $s$ for which the vertices that belong to a same part are consecutive in $s$. 
Such an ordering is called a 
\emph{precedence consistent ordering} (resp. \emph{precedence strongly consistent ordering}) for the given partition.  We define \fpPar{G} (resp. \fpPar{G}) as the minimum value $k$ for which  $G$ is \fp{k} (resp. \fpp{k}). 

The Figure~\ref{fig:a} illustrates a graph that is a \fpp{2} graph. The convention assumed is that the strongly consistent ordering being represented consists of the vertices ordered as they appear in the figure from bottom to top and, for vertices arranged in a same horizontal line, from left to right. Therefore, the strongly consistent ordering represented in Figure~\ref{fig:a} is $s =a,b,c,a',b',c'$.  The graph $C_4$ is not \fpp{2}, despite $\pthin(C_4)=2$. It can be easily verified by brute-force that for all possible bipartitions of its vertex set and for all possible orderings $s$ in which the vertices of a same class are consecutive in $s$, the ordering and the partition are not strongly consistent. On the other hand, a \fpp{k} graph is a proper $k$-thin graph. Therefore, the class of \fpp{k} graphs is a proper subclass of that of proper $k$-thin graphs.

\begin{figure}[htb]
    \centering % <-- added
\includegraphics[width=40mm]{figures/preliminaries/qualiExemplo2FPP.pdf}
%\subfigure[$S_H(X,Y)$]{\label{fig:d}\includegraphics[width=35mm]{exemploSN2FPP.png}}

\caption{A \fpp{2} graph.}
\label{fig:a}
%\label{fig:abcd}
\end{figure}


If a vertex order ${<}$ is given, by Theorem~\ref{thm:coloring-order}, any partition which is precedence (strongly) consistent with ${<}$ is a valid coloring of $G_{<}$ (resp. $\tilde{G}_{<}$) such that, additionally, the vertices on each color class are consecutive according to ${<}$. 
Without loss of generality, the coloring is non-decreasing with respect to the given vertex order. It is easy to prove by induction that a greedy algorithm that starts coloring the vertices with color $1$ and increases by one the color each time the current vertex has a neighbor already
colored with the current color, gives to each vertex the minimum color it can have over all proper non-decreasing colorings. In particular, the algorithm uses the minimum possible number of colors.

%Let us see that a simple greedy algorithm finds such a coloring with the minimum number of color classes: start with color $1$ and color the vertices ordered by ${<}$. In every step, if the vertex to be colored has a neighbor already colored with the current color, move to the next color. It is easy to prove inductively that for any other assignment of colors such that the color classes are ordered and made of consecutive vertices, each vertex receives a color that is greater or equal to the one given by the proposed algorithm. 

%%Should we explain this more? 

In the following sections we will deal with the case where the vertex partition is given and the problem consists of finding the vertex order. From now on, we will then simply call \emph{precedence consistent ordering} (resp. \emph{precedence strongly consistent ordering}) to one that is such for the given partition. 

